GD-COMET: A Geo-Diverse Commonsense Inference Model

With the increasing integration of AI into everyday life, it's becoming crucial to design AI systems that serve users from diverse backgrounds by making them culturally aware. In this paper, we present GD-COMET, a geo-diverse version of the COMET commonsense inference model. GD-COMET goes beyond Western commonsense knowledge and is capable of generating inferences pertaining to a broad range of cultures. We demonstrate the effectiveness of GD-COMET through a comprehensive human evaluation across 5 diverse cultures, as well as extrinsic evaluation on a geo-diverse task. The evaluation shows that GD-COMET captures and generates culturally nuanced commonsense knowledge, demonstrating its potential to benefit NLP applications across the board and contribute to making NLP more inclusive.

==> figures/qualitative_analysis.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/extrinsic-eval.pdf}
    \caption{Attention analysis of commonsense inferences generated by COMET and \model{} for images from GD-VCR from three regions, i.e., Somalia (Africa), India (South Asia), and South Korea (East Asia).} 
    \label{fig:attention-analysis}
\end{figure*}
